PushNet: Efficient and Adaptive Neural Message Passing

Message passing neural networks have recently evolved into a state-of-the-art approach to representation learning on graphs. Existing methods perform synchronous message passing along all edges in multiple subsequent rounds and consequently suffer from various shortcomings: Propagation schemes are inflexible since they are restricted to $k$-hop neighborhoods and insensitive to actual demands of information propagation. Further, long-range dependencies cannot be modeled adequately and learned representations are based on correlations of fixed locality. These issues prevent existing methods from reaching their full potential in terms of prediction performance. Instead, we consider a novel asynchronous message passing approach where information is pushed only along the most relevant edges until convergence. Our proposed algorithm can equivalently be formulated as a single synchronous message passing iteration using a suitable neighborhood function, thus sharing the advantages of existing methods while addressing their central issues. The resulting neural network utilizes a node-adaptive receptive field derived from meaningful sparse node neighborhoods. In addition, by learning and combining node representations over differently sized neighborhoods, our model is able to capture correlations on multiple scales. We further propose variants of our base model with different inductive bias. Empirical results are provided for semi-supervised node classification on five real-world datasets following a rigorous evaluation protocol. We find that our models outperform competitors on all datasets in terms of accuracy with statistical significance. In some cases, our models additionally provide faster runtime.

==> results_table.tex <==
\begin{tabular}{llllllll|llll}
\toprule
{} &      \textbf{GCN} &      \textbf{GAT} &   \textbf{JK-GCN} &   \textbf{JK-GAT} &      \textbf{SGC} &      \textbf{GIN} &    \textbf{APPNP} &  \textbf{PushNet} &       \textbf{PushNet-PTP} &        \textbf{PushNet-PP} &       \textbf{PushNet-TPP} \\
\midrule
\textbf{CiteSeer        } &  $66.98 \pm 1.48$ &  $67.21 \pm 1.43$ &  $65.51 \pm 1.52$ &  $65.78 \pm 1.27$ &  $68.00 \pm 1.09$ &  $65.24 \pm 1.44$ &  $66.67 \pm 2.35$ &  $67.47 \pm 2.04$ &           $67.98 \pm 1.42$ &  $\mathbf{68.80 \pm 1.44}$ &           $67.58 \pm 1.68$ \\
\textbf{Cora            } &  $79.46 \pm 1.60$ &  $80.49 \pm 1.63$ &  $77.90 \pm 1.79$ &  $78.37 \pm 1.78$ &  $78.34 \pm 2.20$ &  $78.75 \pm 1.65$ &  $82.14 \pm 1.29$ &  $82.38 \pm 1.41$ &           $81.64 \pm 1.53$ &           $79.38 \pm 1.62$ &  $\mathbf{82.61 \pm 1.53}$ \\
\textbf{PubMed          } &  $78.17 \pm 1.39$ &  $77.93 \pm 1.50$ &  $77.37 \pm 1.86$ &  $77.63 \pm 2.06$ &  $76.92 \pm 1.77$ &  $77.02 \pm 1.69$ &  $79.27 \pm 3.50$ &  $79.58 \pm 1.33$ &  $\mathbf{79.90 \pm 1.20}$ &           $77.24 \pm 2.02$ &           $79.88 \pm 1.22$ \\
\textbf{Coauthor CS     } &  $89.69 \pm 0.55$ &  $87.66 \pm 0.91$ &  $89.41 \pm 0.63$ &  $90.21 \pm 0.58$ &  $89.37 \pm 0.43$ &  $89.46 \pm 0.70$ &  $88.69 \pm 1.58$ &  $90.45 \pm 0.83$ &           $90.53 \pm 0.48$ &           $88.94 \pm 0.65$ &  $\mathbf{90.67 \pm 0.43}$ \\
\textbf{Coauthor Physics} &  $91.42 \pm 0.79$ &  $91.30 \pm 0.68$ &  $91.46 \pm 0.76$ &     $o.o.m.$ &     $o.o.m.$ &  $91.85 \pm 0.58$ &  $91.87 \pm 0.71$ &  $92.16 \pm 0.69$ &           $92.10 \pm 0.67$ &           $91.73 \pm 0.60$ &  $\mathbf{92.27 \pm 0.59}$ \\
\bottomrule
\end{tabular}

